A tool assisted methodology to harden programs against multi-faults injections

Fault attacks consist in changing the program behavior by injecting faults at run-time in order to break some expected security properties. Applications are hardened against fault attack adding countermeasures. According to the state of the art, applications must now be protected against multi-fault injection. As a consequence developing applications which are robust becomes a very challenging task, in particular because countermeasures can be also the target of attacks. The aim of this paper is to propose an assisted methodology for developers allowing to harden an application against multi-fault attacks, addressing several aspects: how to identify which parts of the code should be protected and how to choose the most appropriate countermeasures, making the application more robust and avoiding useless runtime checks.

==> methodologie.tex <==
Our methodology:

Let $P$ be a program, $M$ a fault model, $O$ an oracle and $\mu$ a fault order:

\begin{enumerate}
\item Run a vulnerability analysis with Lazart:
\begin{itemize}
\item we obtain a set of successful attacks and $I$ a set of initial states attached to these traces
\item we obtain the set of hot spots
\end{itemize}

\item Attacks Selection:
\begin{itemize}
\item We can focus first on non redundant attacks (they must be eliminate) or hot spots with higher score ?
\item  From that we can deduce with type of attack (i.e. which fault model)  must be blocked at which injection points
\end{itemize}

\item Adding protection scheme:

\begin{itemize}
\item We select protection scheme for each IP and their successful fault models from our catalog (catalogue)
and add them
\item we  run a new analysis (ici on a décaler les attaques)
\item we can execute our optimization for remove unnecessary attack (plutôt à la fin)
\end{itemize}

\end{enumerate}

An iterative process (ou bien on gader les attaque d'order $\mu$ ?)

Au pas 3 on devrait avoir des garanties sur les attaques sélectionnées au pas 2

Ici il faudrait montrer qu'on va décaler les attaques (ou bien section d'après, icic on illustre juste la démarche).

=> Illustrer sur un exemple (à trouver)

%On peut aussi montrer qu'on peut adapter à un sous-ensemble de traces choisi (et donc le décalage aussi)

\begin{algorithm}
\caption{Our algorithm for hardening program}\label{alg:cap}
\begin{algorithmic}
\Require $P$
\Ensure $P'$ is more secure.
\State $T \gets$ get\_traces($P$)
\State $SNRA \gets $ filter\_traces($T$) \Comment{SNRA : Successful non-redundant attacks }
\State $P' \gets P$
\If{$SNRA$ is not null} \Comment{SNRA = [[$(ip_{i};fm_{i}),...,(ip_{n};fm_{n})$],$t_{2},t_{3},...,t_{N} $]}
\While{$t_{i} \in SNRA$ is not null}
\If{$ti = (ip_{i},fm_{i})$ is not visited}
\State $cm \gets $catalog($fm_{i}$)
\State $P' \gets$ apply\_cm\_on($P'$,$ip_{i},cm$)
\EndIf
\EndWhile
\EndIf

\end{algorithmic}
\end{algorithm}
            
A catalog property :

$$ \forall fm \in FM \ / \ catalog(fm) = cm_{x} \Rightarrow  \forall cm \in CM \ / \ cm_{x} >_{fm} cm $$

==> related-work.tex <==
\section{Related work}
\label{sec:related-work}

In \cite{} Martin and all also propose an apporach to verify the robustness
of a program, based on Frama-C/WP pluging. 
Here they systematically add  the annotation fault==0 at the end of the 
function that must be robust.  Our proof of protected scheme are more general:
in the sense we impose to preserve the nominal behavior even in présence of harmess
faults. Futhermore we propose a modular approach allowing to prove only once times
the adequacy of countermeasures. 



+ modulaire


+ problème de bien poser les asserions (loupe une des faiblesses)


% Ajouter qqs refs dans l'intro concernant des outils d'analyse de robustesse et/ou des CMs ?
%papier ARES Karine
%A First ISA-Level Characterization of {EM} Pulse Effects on Superscalar
               %Microarchitectures: {A} Secure Software Perspective
%\cite{ProyHBM019}

Two main topics are related to the contributions presented in this paper: 
(fault injection) counter measure analysis, and cost reduction of software runtime checks. 
 
In \cite{Pattabiraman/IFIP09,Pattabiraman/TC12}, Pattabiraman et al. combine model checking and symbolic execution to study if some tests in the program can be suppressed. Those tests are considered as not-faultable.
Use of model checking to verify the effectiveness of a countermeasure against specific fault models has been common \cite{Lalande/ESORICS14,Goubet/CARDIS15,heydemann2019formally}.
Some recent work make use of static analysis to study robustness of protected program against fault injection.
%In \cite{lacombe2021combining}, using a combination of static analysis with Frama-C \cite{framac} and symbolic execution with Lazart \cite{Potet/ICST14}.
Martin et al. proposed in \cite{martin2022verifying} a methodology to verify that some countermeasure checks are effectively protecting the program against multiple fault attacks using test inversion model. They use a specific \textit{mutated} function corresponding to the fault and use static analysis with Frama-C \cite{framac} to ensures that no path can reach specific oracles without a required number of faults.
They were able to automatically detect a vulnerability in the Wookey Bootloader \cite{wookey}, that has been found in \cite{inter_cesti}.

%\subsection{Countermeasure analysis}

As stated in the introduction, although numerous countermeasure schemes have been already
proposed in the literature, their evaluation essentially consisted in showing how effective they are 
to {\em detect} fault injection attacks, but without precisely analyzing how to {\em reduce} their overhead
and potential {\em redundancies} when applied to a whole piece of code. Moreover, most of these analysis 
only consider {\em single fault} injections.  We list below some existing work on such countermeasure evaluations.


    %- une seule faute 
    %- analyse = robustesse (<> trade-off robustesse vs efficacite)
    %- pas d'objectifs "minimiser le cout" ?
    %- papier sur les CM crypto ??
The countermeasure presented in section \ref{subsec:lalande} is analyzed in~\cite{Lalande/ESORICS14} and \cite{HeydemannLB19}.
The correctness of the hardened code and its robustness with respect to C-level {\em single} jump attack faults is proved 
by model-checking for each basic control-flow statement. In~\cite{HeydemannLB19}, a lighter version of this countermeasure 
scheme is proposed to reduce its overhead (at the cost of delaying the attack detection).
However, this variant remains generic, and it is not (automatically) tailored for a precise code example, which could lead 
to further optimizations.  
%- Efficient Design and Evaluation of Counter-Measures
%\cite{Goubet/CARDIS15}
%similar work, formal verif, model-checking, single fault, rien sur optim .. 

The countermeasure scheme mentioned in section \ref{subsec:cfsign} has been initially described in~\cite{Swift}, and its overhead is compared 
to other related schemes on set of benchmarks. There is no discussion about automated way to reduce this overhead, beyond suggesting
that ''only critical parts of the code'' need to be secured. 

\cite{LeHGD18} presents an LLVM based tool allowing to evaluate software resiliency against hardware faults. It relies on the so-called
SWiFi\footnote{Software Implemented Fault Injection} technique, and relies on Klee as a symbolic test execution platform. 
The fault model considered are {\em bit-flip} of the target register of an LLVM computation or load instruction, 
assuming at most {\em one single fault}. A countermeasure mechanism is proposed by means of {\em executable assertions}
on program variables at different code locations to detect ``silent data corruptions''. Experiments are provided on benchmarks, 
showing the results obtained in terms of fault detected, but the question of reducing the number of assertions is not addressed. 

\cite{BreierHL18} focuses on software encoding schemes to protect {\em cryptographic implementations} against physical attacks.
It proposes a metric to evaluate the robustness of an encoding scheme against {\em single} bit flip or instruction skip, together 
with a {\em probabilistic} simulation based evaluation method allowing to provide some robustness {\em vs.} performance trade-offs. 
Hence, it allows the user to select the most appropriate encoding scheme according to the simulation results. 

Finally, \cite{BrancoHKS18} gives an abstract set-theoretic model to evaluate the 
security level brought by a mitigation scheme with respect to a given set of {\em exploits}. 
However, this model relies on a very high-level quantification on ``how much'' 
a mitigation hardens the probability that an exploit occurs (in terms of big ${\cal O}$ notation). 
Although an application example is given in the context of CFI, the granularity of the results obtained are 
far from the ones we can achieve in our approach. 


%\subsection{Reducing the overhead of runtime checks}
Another line of work related to the one presented in this paper is related to the cost reduction of runtime checks in programs. Such checks are added either by the compiler to enforce type safety, or by dedicated 
tools like Valgrind~\cite{ValgrindPaper} or AdSan~\cite{AdSanPaper}, or even by assertions explicitly added by the developer. The execution time overhead induced by these extra lines of code can become quite significant
and eliminating useless checks can provide important gains. Most of the existing work in this direction are based on abstract interpretation techniques (like~\cite{Stulova18}) to statically prove the validity of some assertions allowing to remove the runtime check. However, the techniques used heavily rely on the fact that the program semantic remains unchanged at runtime, which is clearly not the case in our context of fault injection.


\comm{
{\color{blue}
	autres papiers sur la minimisation de dynamic checks ? \\
        (ex: https://cliplab.org/papers/optchk-ppdp2016.pdf) \\
        papiers sur les hyper graphes + ``reduction de clauses'' (c.f. Cristian)
}
}

